SCALE: Towards Whole-Slide Counterfactual Explanations in Cancer Histopathology

Accurate cancer diagnosis depends on histopathological evaluation, in which tumor morphology drives disease classification and therapeutic decision-making. While deep learning models have demonstrated strong performance in predicting diagnostic and prognostic properties from histopathology images, their clinical adoption remains limited by a lack of interpretability. Unlike conventional medical images where diagnostic findings are spatially localized, histopathological images are characterized by complex textural patterns distributed across the entire whole slide image (WSI), making it difficult to explain model predictions through region-based localization alone. Counterfactual explanations offer a promising alternative by asking "what changes in the image could have altered the model prediction." To achieve this, we propose SCALE, a framework for generating such counterfactual explanations for histopathological DL models. Across nine counterfactual directions spanning multiple cancer types, SCALE generates counterfactual explanations that consistently shift model predictions toward the intended diagnostic target while maintaining biological feasibility. In a blinded review by pathologists, SCALE demonstrated superior morphological plausibility compared to baseline methods (win rate of 91.7%) and robust counterfactual effectiveness (target consistency of 96.7%). These results suggest that SCALE generates morphologically plausible and effective counterfactual explanations that can be applied to improve the interpretability of deep learning models for histopathology.

==> resources/packages.tex <==
% For flexible citation formats (author-year, numeric)
\usepackage{natbib}

% For UTF-8 encoded CJK (Chinese, Japanese, Korean) characters
\usepackage{CJKutf8}

%\newcommandx
\usepackage{xargs}  

% todo notes
\usepackage{todonotes}  

% multirow
\usepackage{multirow}


% cref
\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}

% % using itemize
% \usepackage{enumerate}


\usepackage{subcaption}


\usepackage{svg}

